Probabilistic Routing for Graph-Based Approximate Nearest Neighbor Search

Approximate nearest neighbor search (ANNS) in high-dimensional spaces is a pivotal challenge in the field of machine learning. In recent years, graph-based methods have emerged as the superior approach to ANNS, establishing a new state of the art. Although various optimizations for graph-based ANNS have been introduced, they predominantly rely on heuristic methods that lack formal theoretical backing. This paper aims to enhance routing within graph-based ANNS by introducing a method that offers a probabilistic guarantee when exploring a node's neighbors in the graph. We formulate the problem as probabilistic routing and develop two baseline strategies by incorporating locality-sensitive techniques. Subsequently, we introduce PEOs, a novel approach that efficiently identifies which neighbors in the graph should be considered for exact distance calculation, thus significantly improving efficiency in practice. Our experiments demonstrate that equipping PEOs can increase throughput on commonly utilized graph indexes (HNSW and NSSG) by a factor of 1.6 to 2.5, and its efficiency consistently outperforms the leading-edge routing technique by 1.1 to 1.4 times.

==> discussion.tex <==
\subsection{Computational Cost}
\label{sec:discussion}
%\subsection{Implementation and Updates} 
%In practice, to avoid storing the pair ($w_{reg}, w_{res}$) for every data point and to save some computational cost, we can alternatively compute an average pair $\bar w_{reg}, \bar w_{res}$ and apply it to every edge. In fact, if $w_{res}$ is small and varies in a small domain, such simplification has little impact on the distribution in~\eqref{eq:N_ex_min}. 

%Next, we discuss the updates of PEOs. Since PEOs only stores the information of edges, we only need to accordingly add or delete such information if any insertion/deletion of edge occurs. More importantly, since we generate all the projected vectors randomly, PEOs is not sensitive to the change of data distribution. 

% We analyze the time and space cost of PEOs and leave the discussion on the comparison with quantization in Appendix~\ref{sec:quantization}. 

For $H(\bm{e})$, we need at most two multiplications, $L+1$ additions and $L+1$ reads to get $H(\bm{e})$. For $T_{r}(\bm{e})$, we need one addition, one read, two subtractions and two divisions since all the inner products and $F^{-1}_{\bm{e},\epsilon}(\cdot)$ can be obtained directly by the pre-computed tables. 
% Noting that the whole procedure of PEOs test can be greatly accelerated by SIMD (16 edges are tackled simultaneously), which makes the estimation time much shorter than the original exploration time (Particularly, since the raw vectors of neighbors are stored separately in the memory, loading them into CPU is quite costly.). 
On the other hand, by using PEOs, \#exact-distance-computation can be reduced by 70\% -- 80\%, as shown in Appendix~\ref{sec:distance-reall-curves}. 

As for the space cost, for every edge, we need $L+1$ bytes for vector id's, three bytes for weights, and two bytes or four bytes for $\left\| \bm{u} \right\|^2 / 2$ and $\left\| \bm{e} \right\|$, where the scalar quantization is used here. Such space cost is affordable for 10M-scale and smaller datasets on a single PC (Appendix~\ref{sec:index-size-and-time}). For 100M-scale and larger datasets, we can sacrifice a little efficiency to significantly reduce the space cost (Appendix~\ref{sec:100M}). 

 

==> ethics.tex <==
\section*{Impact Statement}
In this paper, we studied ANNS, a fundamental problem in the area of machine learning. The proposed routing test algorithm can be plugged into current graph indexes for ANNS. To the best of our knowledge, there is no negative societal impact related to this research. 
